True2F: Backdoor-resistant authentication tokens

We present True2F, a system for second-factor authentication that provides the benefits of conventional authentication tokens in the face of phishing and software compromise, while also providing strong protection against token faults and backdoors. To do so, we develop new lightweight two-party protocols for generating cryptographic keys and ECDSA signatures, and we implement new privacy defenses to prevent cross-origin token-fingerprinting attacks. To facilitate real-world deployment, our system is backwards-compatible with today's U2F-enabled web services and runs on commodity hardware tokens after a firmware modification. A True2F-protected authentication takes just 57ms to complete on the token, compared with 23ms for unprotected U2F.

==> main.tex <==
\input{preamble}

\begin{document}


\title{True2F: Backdoor-resistant authentication tokens\\
{\normalsize {\normalfont \today}}} 
\author{Emma Dauterman\\
\textit{Stanford and Google}
\and
Henry Corrigan-Gibbs\\
\textit{Stanford}
\and
David Mazi\`eres\\
\textit{Stanford}
\and
Dan Boneh\\
\textit{Stanford}
\and
Dominic Rizzo\\
\textit{Google}
}
\maketitle
%\thispagestyle{empty}

\frenchspacing
\input{abs}
\input{intro}
\input{bg}
\input{goals}
\input{crypto}
\input{count}
\input{protocol}
\input{impl}
\input{eval}
\input{rel}
\input{concl}

%\clearpage
{\small
\setstretch{0.95}
\bibliography{refs}
\bibliographystyle{abbrv} 
}

\appendix
\input{failure}
\input{ecdsa}
\input{sig}
\input{keygen}
\input{san}


\end{document}

